Dark Matter and Fundamental Physics Searches with IACTs

Cosmic gamma rays are a valid probe to search for fundamental physics. Some of these exotic and exciting scenarios are the subject of this contribution to the book. All current Imaging Atmospheric Cherenkov Telescopes (IACTs) have invested a great deal of time and resources in scouting these out. In this chapter, we focus on the case of indirect search for weakly interacting massive particles (Sec. 8.1) and that of search for axion-like particles (Sec. 8.2). We continue with less debated, yet interesting studies on the search for primordial black holes (Sec. 8.3), tau-neutrinos (8.4), and magnetic monopoles (8.5). Other scenarios of fundamental physics like the search for Lorentz Invariance violations are treated elsewhere in the book. We structured the contribution providing a self-contained (yet minimal) theoretical framework, as well as a complete report of all IACTs' published contribution to the topics under consideration (updated until 2022). Our aim is to provide a reference review as well as take a photograph of the effort of the current generation of IACTs and the challenges taken, in preparation of the next-generation instrument to come, the Cherenkov Telescope Array.

==> add/acro.tex <==
\newacronym{agn}{AGN}{Active Galactic Nucleus}
\newacronym{alp}{ALP}{\textit{axion-like} particle}
\newacronym{ashra}{ASHRA}{All-sky Survey High Resolution Air-shower detector}
\newacronym{bh}{BH}{black hole}
\newacronym{cdm}{CDM}{Cold Dark Matter}
\newacronym{cmb}{CMB}{Cosmic Microwave Background}
\newacronym{cmz}{CMZ}{Central Molecular Zone}
\newacronym{cp}{CP}{Charge-Parity}
\newacronym{cr}{CR}{Cosmic Ray}
\newacronym{cta}{\cta}{Cherenkov Telescope Array}
\newacronym{dm}{DM}{Dark Matter}
\newacronym[longplural={Dwarf Spheroidal Galaxies}]{dsph}{dSph}{Dwarf Spheroidal Galaxy}
\newacronym{ebl}{EBL}{Extragalactic Background Light}
\newacronym{fov}{F.O.V.}{field of view}
\newacronym{fsrq}{FSRQ}{Flat Spectrum Radio Quasar}
\newacronym{gc}{GC}{Galactic Centre}
\newacronym{grand}{GRAND}{Giant Radio Array for Neutrino Detection}
\newacronym{grb}{GRB}{Gamma-ray Burst}
\newacronym{guts}{GUTs}{Grand Unification Theories}
\newacronym{hawc}{HAWC}{High Altitude Water Cherenkov Experiment}
\newacronym{hess}{H.E.S.S.}{High Energy Stereoscopic System }
\newacronym{iact}{IACT}{Imaging Atmospheric Cherenkov Telescope}
\newacronym{icm}{ICM}{Intra-Cluster Medium}
\newacronym{imbh}{IMBH}{Intermediate Mass Black Hole}
\newacronym{lhaaso}{LHAASO}{Large High Altitude Air Shower Observatory}
\newacronym{lsp}{LSP}{lightest supersymmetric particle}
\newacronym{lst}{LST}{Large Size Telescope}
\newacronym{machos}{MACHOs}{massive astrophysical compact halo objects}
\newacronym{MAGIC}{MAGIC}{Major Atmospheric Gamma-ray Imaging Cherenkov}
\newacronym{magic}{MAGIC}{Major Atmospheric Gamma-ray Imaging Cherenkov}
\newacronym{mc}{MC}{Monte Carlo}
\newacronym{mm}{MM}{magnetic monopole}
\newacronym{mms}{MMs}{magnetic monopoles}
\newacronym{mw}{MW}{Milky Way}
\newacronym{MoG}{MoG}{Modified Gravity}
\newacronym{MoND}{MoND}{Modified Newtonian Dynamics}
\newacronym{nfw}{NFW}{Navarro-Frenk-White}
\newacronym{ns}{NS}{neutron star}
\newacronym{qcd}{QCD}{quantum chromodynamics}
\newacronym{pao}{PAO}{Pierre Auger Observatory}
\newacronym{pbh}{PBH}{primordial black hole}
\newacronym{poemma}{POEMMA}{Probe of Extreme Multi-Messenger Astrophysics}
\newacronym{pmt}{PMT}{photomultiplier tube}
\newacronym{pwn}{PWNe}{pulsar wind nebulae}
\newacronym{rf}{RF}{Random Forest}
\newacronym{sm}{SM}{Standard Model}
\newacronym{sn}{SN}{supernova}
\newacronym{snr}{SNR}{supernova remnant}
\newacronym{susy}{SUSY}{Super-Symmetry}
\newacronym{swgo}{SWGO}{Southern Wide-field Gamma-ray Observatory}
\newacronym{veritas}{VERITAS}{Very Energetic Imaging Telescope Array System}
\newacronym{vhe}{VHE}{very-high-energy}
\newacronym{wimp}{WIMP}{weakly interacting massive particle}


\usepackage{amsthm}

%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{exercise}[theorem]{Exercise}

\newenvironment{myboxedtext}[1]
  {\begin{eBox}\textcolor{ocre}{{\bfseries\small\sffamily#1~}}}
  {\hfill{\color{ocre}\tiny\ensuremath{\blacksquare}}\end{eBox}}        








==> add/settings.tex <==
\usepackage{comment}% added by M. Doro
\usepackage{longtable,caption}
\usepackage{enumitem} % Michele 

%DIF PREAMBLE EXTENSION ADDED BY LATEXDIFF
%DIF UNDERLINE PREAMBLE %DIF PREAMBLE
\RequirePackage[normalem]{ulem} %DIF PREAMBLE
\RequirePackage{color}\definecolor{RED}{rgb}{1,0,0}\definecolor{BLUE}{rgb}{0,0,1} %DIF PREAMBLE
\providecommand{\DIFadd}[1]{{\protect\color{blue}\uwave{#1}}} %DIF PREAMBLE
\providecommand{\DIFdel}[1]{{\protect\color{red}\sout{#1}}}                      %DIF PREAMBLE
%DIF SAFE PREAMBLE %DIF PREAMBLE
\providecommand{\DIFaddbegin}{} %DIF PREAMBLE
\providecommand{\DIFaddend}{} %DIF PREAMBLE
\providecommand{\DIFdelbegin}{} %DIF PREAMBLE
\providecommand{\DIFdelend}{} %DIF PREAMBLE
%DIF FLOATSAFE PREAMBLE %DIF PREAMBLE
\providecommand{\DIFaddFL}[1]{\DIFadd{#1}} %DIF PREAMBLE
\providecommand{\DIFdelFL}[1]{\DIFdel{#1}} %DIF PREAMBLE
\providecommand{\DIFaddbeginFL}{} %DIF PREAMBLE
\providecommand{\DIFaddendFL}{} %DIF PREAMBLE
\providecommand{\DIFdelbeginFL}{} %DIF PREAMBLE
\providecommand{\DIFdelendFL}{} %DIF PREAMBLE
%DIF END PREAMBLE EXTENSION ADDED BY LATEXDIFF


\usepackage{verbatim} % added by M. Doro
\usepackage[acronym]{glossaries}
\usepackage{graphicx}
%\usepackage{natbib}
\usepackage{mathtools, cuted}
\usepackage{amsmath,amssymb,esint}
\usepackage[sort&compress,comma,authoryear]{natbib}
\usepackage[colorlinks=true,allcolors=blue,bookmarks=true]{hyperref}

% ADDED BY MICHELE, MIGUEL


\newcommand{\gammaray}{gamma-ray}
\newcommand{\hess}{H.E.S.S.}
\newcommand{\hegra}{HEGRA}
\newcommand{\cta}{CTA}
\newcommand{\LAT}{\emph{Fermi}-LAT}
\newcommand{\xmm}{\emph{XMM}-Newton}
\newcommand{\chandra}{\emph{Chandra}}
\newcommand{\nustar}{\emph{NuStar}}
\newcommand{\apj}{ApJ}
\newcommand{\apjs}{ApJS}
\newcommand{\apjf}{The Astrophysical Journal}
\newcommand{\apjl}{ApJL}
\newcommand{\apjlf}{The Astrophysical Journal Letters}
\newcommand{\aap}{A\&A}
\newcommand{\aapf}{Astronomy \& Astrophysics}
\newcommand{\aapr}{A\&A~Rev.}
\newcommand{\apss}{Ap\&SS}
\newcommand{\aaprf}{Astronomy \& Astrophysics Reviews}
\newcommand{\araa}{Annual Rev. of Astron. and Astrophys.}
\newcommand{\araaf}{Annual Review of Astronomy and Astrophysics}
\newcommand{\nat}{Nature}
\newcommand{\science}{Science}
\newcommand{\ap}{Astrop. Phys. }
\newcommand{\apf}{Astroparticle Physics Journal }
%\newcommand{\ajf}{Astroparticle Journal}
\newcommand{\ijmpd}{Int. J. of Mod. Phys. D}
\newcommand{\ijmpdf}{International Journal of Modern Physics D}
\newcommand{\jcap}{J. Cosmology Astropart. Phys.}
\newcommand{\jcapf}{Journal of Cosmology and Astroparticle Physics}
\newcommand{\jhea}{J. High-Energy Astroph.}
\newcommand{\jheaf}{Journal of High Energy Astrophysics}
\newcommand{\mnras}{MNRAS}
\newcommand{\mnrasf}{Monthly Notices of the Royal Astronomical Society}
\newcommand{\nima}{Nucl. Instrum. and Meth. in Phys. Research A}
\newcommand{\nimaf}{Nuclear Instruments and Methods in Physics Research A}
\newcommand{\plb}{Phys. Let. B}
\newcommand{\plbf}{Physics Letter B}
\newcommand{\prd}{Phys.~Rev.~D}
\newcommand{\prdf}{Physical Review D}
\newcommand{\prl}{Phys.~Rev.~Letter}
\newcommand{\prlf}{Physical Review Letter}
\newcommand{\physrep}{Physics Reports}
\newcommand{\pasj}{Pub. of the ASJ}
\newcommand{\pasjf}{Publications of the Astronomical Society of Japan}
\newcommand{\pos}{PoS}
\newcommand{\posf}{Proc. of Science}
\newcommand{\ssr}{S Review}
\newcommand{\etal}{\emph{et al.}}
\newcommand{\coll}{Collaboration}
%% RM's definitions (to be removed later)
\def\be{\begin{equation}}
\def\ee{\end{equation}}
\def\bea{\begin{eqnarray}}
\def\eea{\end{eqnarray}}
\def\beas{\begin{eqnarray*}}
\def\eeas{\end{eqnarray*}}
\def\lb{\label}
\def\bom{\mbox{\boldmath $\omega$}}
\def\bphi{\mbox{\boldmath $\phi$}}
\def\bna{\mbox{\boldmath $\nabla$}}
\def\brho{\mbox{\boldmath $\rho$}}
\def\lie{\mbox{\pounds}}
\def\la{\langle}
\def\ra{\rangle}
\def\pa{\partial}
\def\sq{\sqrt }
\def\l{\lambda }
\def\ph{\phi }
\def\o{\omega}
\def\t{\tau }
\def\th{\theta }
\def\k{\kappa }
\def\p{\pi }
\def\Ph{\Phi }
\def\ps{\psi }
\def\Ps{\Psi }
\def\ch{\chi }
\def\d{\delta }
\def\a{\alpha}
\def\e{\epsilon }
\def\b{\beta}
\def\do{\dot }
\def\dag{\dagger }
\def\pr{\prime }
\def\ve{\vert }
\def\hsp5{\hspace{5mm}}
\def\h{\hat }
\def\dag{\dagger }
\def\bp{\begin{pmatrix}}
\def\ep{\end{pmatrix}}
\def\bv{\begin{vmatrix}}
\def\ev{\end{vmatrix}}
\def\ran{\rangle }
\def\lan{\langle }
\def\half{\frac {1}{2}}
\def\kno{\vert n^{(0)}\ran }
\def\bno{\lan n^{(0)} \vert }


\usepackage{colortbl}
\usepackage{esvect}
\newcommand{\aaa}{alpha}
\newcommand{\svUL}{\langle \sigma \mathit{v} \rangle^\mathrm{UL}}
\newcommand{\sv}{\langle \sigma \mathit{v} \rangle}
\newcommand{\svsvt}{\sv_\mathrm{svt}}
\newcommand{\svdsu}{\sv_{2.71}}
\newcommand{\aaasvt}{\aaa_\mathrm{svt}}
\newcommand{\aaadsu}{\aaa_{2.71}}
\newcommand{\hataaa}{\hat{\aaa}}
\newcommand{\hatsv}{\widehat{\langle \sigma \mathit{v} \rangle}}
\newcommand{\doublehatnu}{\doublehat{\bm{\nu}}}
\newcommand{\hatnu}{\hat{\bm{\nu}}}
\newcommand{\hatmu}{\hat{\bm{\mu}}}
\newcommand{\hattheta}{\hat{\bm{\theta}}}
\newcommand{\thetaann}{\theta_\mathrm{ann}}
\newcommand{\thetadec}{\theta_\mathrm{dec}}
\newcommand{\data}{\bm{\mathcal{D}}}
\newcommand{\lkl}{\mathcal{L}}
%\newcommand{\loglkl}{\mathcal{l}}
\newcommand{\loglkl}{\log\mathcal{L}}
\newcommand{\overbar}[1]{\mkern 3.5mu\overline{\mkern-3.5mu#1\mkern-3.5mu}\mkern 3.5mu}
\newcommand{\non}{{N_\mathrm{ON}}}
\newcommand{\noff}{{N_\mathrm{OFF}}}
\newcommand{\emin}{{E'_\mathrm{min}}}
\newcommand{\emax}{{E'_\mathrm{max}}}
\newcommand{\mdm}{m_\mathrm{DM}}
\newcommand{\tdm}{\tau_\mathrm{DM}}
\newcommand{\taudm}{\tau_\mathrm{DM}}
\newcommand{\tdmLL}{\tau_\mathrm{DM}^\mathrm{UL}}
\newcommand{\dom}{{\Delta\Omega}}
\newcommand{\aeff}{ A_\mathrm{eff}}
\newcommand{\barJ}{\bar{J}}
\newcommand{\bb}{b\bar{b}}
\newcommand{\WW}{W^+W^-}
\newcommand{\tautau}{\tau^+\tau^-}
\newcommand{\mumu}{\mu^+\mu^-}
\newcommand{\gammagamma}{\gamma\gamma}
\newcommand{\Jobs}{J_\mathrm{obs}}
\newcommand{\Jobsi}{J_\mathrm{obs,i}}
\newcommand{\Dobs}{D_\mathrm{obs}}
\newcommand{\Dobsi}{D_\mathrm{obs,i}}
\newcommand{\lp}{\lambda_P}
\newcommand{\Junits}{GeV$^2$ cm$^{-5}$}
\newcommand{\Jdecunits}{GeV cm$^{-2}$}
\newcommand{\svunits}{cm$^3$ s$^{-1}$}
\newcommand{\Fermi}{\textit{Fermi}\xspace}
\newcommand{\Tobsi}{T_{\mathrm{obs},i}}
\newcommand{\triangulum}{Tri~II\xspace}
\newcommand{\ppterm}{\frac{d\overline{\Phi}_\textrm{PP}}{dE}}
\newcommand{\ppdecterm}{\frac{d\overline{\Phi}_\textrm{PP,dec}}{dE}}
\newcommand{\sppterm}{d\overline{\Phi}_\textrm{PP}/dE}
\newcommand{\sigmaJ}{\sigma_J}
\newcommand{\Nonij}{{N_{\mathrm{ON},ij}}}
\newcommand{\Noffij}{{N_{\mathrm{OFF},ij}}}
\newcommand{\Nbins}{N_\mathrm{bins}}
\newcommand{\gij}{g_{ij}}
\newcommand{\goffij}{g_{ij}^{OFF}}
\newcommand{\bij}{b_{ij}}
\newcommand{\fij}{f_{ij}}
\newcommand{\tauobsi}{\kappa_{\mathrm{obs},i}}
\newcommand{\sigmataui}{\sigma_{\kappa,i}}
\newcommand{\sigmatausys}{\sigma_{\kappa}^{sys}}
\newcommand{\sigmataustat}{\sigma_{\kappa}^{stat}}
%%% OLD
\newcommand{\Eminj}{{E'_{\mathrm{min},j}}}
\newcommand{\Emaxj}{{E'_{\mathrm{max},j}}}
%%% NEW
\newcommand{\epMinj}{{E'_{\mathrm{min},j}}}
\newcommand{\epMaxj}{{E'_{\mathrm{max},j}}}
%%%
\newcommand{\MNRAS}{Mon. Not. Roy. Astron. Soc. }
%\newcommand{\Comment}[1]{{\color{red}{#1}}}
\newcommand{\atot}{ A_\mathrm{tot}}
\newcommand{\eff}{\epsilon}
\newcommand{\psf}{\mbox{Point Spread Function}}
\newcommand{\bpt}{\bp_\mathrm{tel}}
\newcommand{\bps}{\bp_\mathrm{src}}
\newcommand{\pdfE}{f_E}
\newcommand{\pdfP}{{f_\bp}}
\newcommand{\pdfTheta}{f_\theta}
\newcommand{\fluxunits}{cm$^{-2}$ s$^{-1}$ TeV$^{-1}$}
\newcommand{\difffluxunits}{\fluxunits\, sr$^{-1}$}
\newcommand{\taui}{\tau_i}
\newcommand{\muij}{\mu_{ij}}
\newcommand{\tauij}{\tau_{ij}}
\newcommand{\kij}{\kappa_{ij}}
\newcommand{\RiCR}{R_i^\mathrm{CR}}
\newcommand{\RiX}{R_i^\mathrm{X}}
\newcommand{\RiGDE}{R_i^\mathrm{GDE}}
\newcommand{\Rmin}{R_\mathrm{min}}
\newcommand{\Rmax}{R_\mathrm{max}}
\newcommand{\RminCR}{R_\mathrm{min}^\mathrm{CR}}
\newcommand{\RmaxCR}{R_\mathrm{max}^\mathrm{CR}}
\newcommand{\RminGDE}{R_\mathrm{min}^\mathrm{GDE}}
\newcommand{\RmaxGDE}{R_\mathrm{max}^\mathrm{GDE}}
\newcommand{\dNdE}{\frac{dN}{dE}}
\newcommand{\dJdp}{\frac{dJ}{d\Omega}}
\newcommand{\dJdpp}{\frac{dJ}{d\Omega'}}
\newcommand{\Jann}{J_\mathrm{ann}}
\newcommand{\Jdec}{J_\mathrm{dec}}
\newcommand{\dJdecdpp}{\frac{dJ_\mathrm{dec}}{d\Omega'}}
\newcommand{\Jannsmooth}{\bar{J}_\mathrm{ann}}
\newcommand{\dJdpann}{\frac{d\Jann}{d\Omega}}
\newcommand{\dJdthetaann}{\frac{d\Jann}{d\theta}}
\newcommand{\dJdpdec}{\frac{d\Jdec}{d\Omega}}
\newcommand{\diffJunits}{\Junits\, sr$^{-1}$}
\newcommand{\Dunits}{GeV cm$^{-2}$}
\newcommand{\diffDunits}{\Dunits\, sr$^{-1}$}
\newcommand{\rhounits}{GeV cm$^{-3}$}
\newcommand{\ttbar}{t\bar{t}}
\newcommand{\Nbk}{b}
\newcommand{\Noff}{N_\mathrm{OFF}}
\newcommand{\Non}{N_\mathrm{ON}}
\newcommand{\Rbk}{\frac{d\bar{b}}{dtdE'd\bp'}}
\newcommand{\Roff}{\frac{dN_\mathrm{OFF}}{dtdE'}}
\newcommand{\Tobs}{T_\mathrm{obs}}
\newcommand{\Emin}{E_\mathrm{min}}
\newcommand{\Emax}{E_\mathrm{max}}
\newcommand{\Emini}{{E_{\mathrm{min},i}}}
\newcommand{\Emaxi}{{E_{\mathrm{max},i}}}
%\newcommand{\hatsv}{\widehat{\langle \sigma \mathit{v} \rangle}}
%\newcommand{\hatnu}{\hat{\bm{\nu}}}
%\newcommand{\data}{\bm{\mathcal{D}}}
\newcommand{\NEbins}{N_{E'}}
\newcommand{\NPbins}{N_{\bp'}}
%\newcommand{\gij}{g_{ij}}
%\newcommand{\bij}{b_{ij}}
\newcommand{\bijCR}{b_{ij}^\mathrm{CR}}
\newcommand{\bijGDE}{b_{ij}^\mathrm{GDE}}
\newcommand{\bijX}{b_{ij}^\mathrm{X}}
%\newcommand{\Nonij}{{N_{\mathrm{ON},ij}}}
\newcommand{\Nij}{{N_{ij}}}
%\newcommand{\Noffij}{{N_{\mathrm{OFF},ij}}}
%\newcommand{\Jobs}{J_\mathrm{obs}}
\newcommand{\tauobs}{\tau_\mathrm{obs}}
%\newcommand{\sigmaJ}{\sigma_J}
\newcommand{\sigmatau}{\sigma_\tau}
\newcommand{\sigmak}{\sigma_\kappa}
\newcommand{\tauDM}{\tau_\mathrm{DM}}
\newcommand{\tauDMSen}{\tau_\mathrm{DM|2.71}}
\newcommand{\FoV}{\mbox{FoV}}
\newcommand{\GeV}{\mbox{GeV}}
\newcommand{\TeV}{\mbox{TeV}}
\newcommand{\muG}{\mu\mbox{G}}
\newcommand{\nutau}{$\nu_\tau$~}
\newcommand{\nutaus}{$\nu_\tau$s~}

\usepackage{lineno}
%\linenumbers


\usepackage{fullpage}

\input{add/acro.tex}
\makeglossaries
